Proof-of-Prestige: A Useful Work Reward System for Unverifiable Tasks

As cryptographic tokens and altcoins are increasingly being built to serve as utility tokens, the notion of useful work consensus protocols, as opposed to number-crunching PoW consensus, is becoming ever more important. In such contexts, users get rewards from the network after they have carried out some specific task useful for the network. While in some cases the proof of some utility or service can be proved, the majority of tasks are impossible to verify. In order to deal with such cases, we design Proof-of-Prestige (PoP) - a reward system that can run on top of Proof-of-Stake blockchains. PoP introduces prestige which is a volatile resource and, in contrast to coins, regenerates over time. Prestige can be gained by performing useful work, spent when benefiting from services and directly translates to users minting power. PoP is resistant against Sybil and Collude attacks and can be used to reward workers for completing unverifiable tasks, while keeping the system free for the end-users. We use two exemplar use-cases to showcase the usefulness of PoP and we build a simulator to assess the cryptoeconomic behaviour of the system in terms of prestige transfer between nodes.

==> sections/acknowledgements.tex <==
\section*{Acknowledgements}
Michał Król is supported by the EC H2020 ICN2020 project under grant agreement number 723014, Alberto Sonnino is supported by the EU H2020 DECODE project under grant agreement number 732546, Mustafa Al-Bassam is supported by a scholarship from The Alan Turing Institute, and Ioannis Psaras is supported by the EPSRC INSP Early Career Fellowship under grant agreement number EP/M003787/1.
Many thanks to Sheharbano for helpful suggestions on early manuscripts.

==> sections/background.tex <==
\section{Background}
We present backgrounds on composite signatures and Proof-of-Stake.

\yiannis{Text below comes out of the blue :) For each of the subsections we need to very briefly say how we use the concepts discussed, or what are their problems and why they need improvement, e.g., what is the problem of \pos and therefore we need \pop? Rich get richer - anything else? Is it unfit for some scenarios?}

% ================
\subsection{Composite Signatures}
Composite signatures~\cite{saxena2014increasing} are aggregate signatures satisfying the properties of \first \emph{incremental composition}, \second \emph{one-way}, and \third \emph{no-ordering}. \emph{Incremental composition} means that a number of individual signatures can be combined into a single signature, and more signatures can be added to the composite at any time; \emph{one-way} refers to the computational difficulty to obtain any sub-composite of signatures from only the composite signature; and \emph{no-ordering} means that the signature does not maintain order.

We adopt the definition of composite signature schemes given by Saxena~\etal~\cite{saxena2014increasing}. Let's consider a message-descriptor $l$ made of pairs of (message,verification key): $l = \{(m_1 ,vk_1 ), \dots , (m_i ,vk_i )\}$. A composite signature scheme $\textbf{SIG}$ is defined by the set of algorithms below:
\begin{itemize}
\item \functiondef{SIG.Setup($1^\lambda$)}{$params$} defines the system parameters $params$ with respect to the security parameter $\lambda$. These parameters are publicly available.

\item \functiondef{SIG.Gen($params$)}{$sk,vk$} generates their secret key $sk$ and verification key $vk$ from the public $params$.

\item \functiondef{SIG.Sign($sk,m$)}{$\sigma$} outputs a single signature $\sigma$ on the message $m$ computed from the secret key $sk$.

\item \functiondef{SIG.Verify($l,\sigma$)}{$b$} takes as input a message-descriptor $l$ and a signature $\sigma$. Outputs a decision bit $b$ about the validity of the signature if all the messages in $l$ are unique; otherwise, it produces output: $invalid$.

\item \textbf{SIG.Compose} takes as input two pairs of (message-descriptors,signatures), $(l_1 ,\sigma_1 )$ and $(l_2 ,\sigma_2)$. If \algo{Sig.Verify($l_1,\sigma_1$)} = \algo{Sig.Verify($l_2,\sigma_2$)} = $valid$ and $l_1 \cap l_2 = \emptyset$, this scheme outputs the composite signature $\sigma$ on the message descriptors $l_1 \cap l_2$; otherwise it produces output: $\perp$. 
\end{itemize}

%An interesting property of composite signatures is that an adversary cannot extract any individual signature from a composite signature~\cite{saxena2014increasing}.

Saxena~\etal~\cite{saxena2014increasing} propose a provably secure composite signature scheme but whose signature size increases linearly with the number of compositions. They also posit that BGLS signatures~\cite{bgls} are secure under a weaker security assumption~\cite{saxena2014increasing}. In the rest of the paper, we use BGLS as composite signature scheme as its signature size remains constant with the number of compositions.
\alberto{@Alberto, justify why we are happy with weaker security (the answer is at end of section 7 of~\cite{saxena2014increasing})}

% ================
\subsection{Proof of stake}
Proof-of-Stake (\pos) is an alternative consensus mechanism to Proof-of-Work that is less energy intensive, where instead of the amount of computing power that participants have used to determine their likelihood of producing blocks, the amount of stake they have in the system (\ie coins) is used to determine their likelihood of producing blocks.

In \pos, participants vote on new blocks weighted by their in-band investment such as the amount of currency
held in the blockchain. A number of recent systems have provably secure \pos protocols \cite{bentov2016snow, david2017ouroboros, kiayias2017ouroboros}. A common
theme in these systems is to randomly elect a leader from among the stakeholders, which then appends a block to the blockchain. Leader election may be public, that is, the outcome is visible to all the participants \cite{bentov2016snow} \cite{kiayias2017ouroboros}.


==> sections/discussion.tex <==
\section{Discussion}\label{sec:compatibility}
As previously stated, \pop is not a new consensus protocol, but a mechanism of assigning minting power to users with existing \pos protocols. As prestige is a volatile resource, it cannot be used with \pos protocols which require stakers to deposit and lock their coins for a long period of time (such as Casper FFG~\cite{casper}), so that their deposit can be reduced if they are caught misbehaving. This is because prestige cannot be locked, as by design it automatically increases or decreases. However, it is compatible with protocols such as Ouroboros \cite{kiayias2017ouroboros} which do not require deposits, and adapt to the new stake mapping in the system every epoch, where coins (and prestige) do not have to be locked up and can be transferred at any time.

\michal{We probably need a security analysis section. We should think how PoP is changing the whole security model of PoS. What about long range attacks etc. }


==> sections/security.tex <==
\section{Security Considerations}

\michal{Add discussion about how our design changes resistance to PoS/PoW attacks}

